ByzSFL: Achieving Byzantine-Robust Secure Federated Learning with Zero-Knowledge Proofs

The advancement of AI models, especially those powered by deep learning, faces significant challenges in data-sensitive industries like healthcare and finance due to the distributed and private nature of data. Federated Learning (FL) and Secure Federated Learning (SFL) enable collaborative model training without data sharing, enhancing privacy by encrypting shared intermediate results. However, SFL currently lacks effective Byzantine robustness, a critical property that ensures model performance remains intact even when some participants act maliciously. Existing Byzantine-robust methods in FL are incompatible with SFL due to the inefficiency and limitations of encryption operations in handling complex aggregation calculations. This creates a significant gap in secure and robust model training. To address this gap, we propose ByzSFL, a novel SFL system that achieves Byzantine-robust secure aggregation with high efficiency. Our approach offloads aggregation weight calculations to individual parties and introduces a practical zero-knowledge proof (ZKP) protocol toolkit. This toolkit supports widely used operators for calculating aggregation weights, ensuring correct computations without compromising data privacy. Not only does this method maintain aggregation integrity, but it also significantly boosts computational efficiency, making ByzSFL approximately 100 times faster than existing solutions. Furthermore, our method aligns with open-source AI trends, enabling plaintext publication of the final model without additional information leakage, thereby enhancing the practicality and robustness of SFL in real-world applications.

==> old/2.tex <==
\section{Background}
\label{sec:Background}


\subsection{FL and Secure Aggregation for FL}
\label{subsec:FL and Secure Aggregation for FL}
% 联邦学习 (FL) 是一种分布式设置~\cite{}，在这种设置中，多个客户端在中央服务器的协调下协作学习一个模型。在FL的每一轮中，(1) 服务器会将当前模型广播给该轮中参与的所有客户端。然后，在(2) 本地训练步骤中，客户端使用各自的本地数据集更新模型。最后，客户端进入(3) 聚合步骤，在该步骤中，所有本地训练的模型都会进行预处理并聚合到服务器，以获得更新后的模型。这些步骤 (1-3) 会在多个训练轮次中反复迭代。
Federated Learning (FL) is a distributed framework~\cite{zhu2020privacy,zhang2021survey,xu2021federated} in which multiple clients collaboratively learn a model under the coordination of a central server. In each round of FL, first the server broadcasts the current model to all clients participating in that round. Then, second step, a local training step, clients update the model using their own local datasets. Finally, the third step, the clients proceed to an aggregation step, where all locally trained models are pre-processed and aggregated by the server to obtain an updated model. These steps (1-3) are repeated over several training rounds.



% 在上述步骤 (3) 中，安全聚合的作用，也是这一步在secure Federated learning (SFL) 和 Federated Learning 中存在主要区别，在这一步, 对于secure Federated learning, 他会使用 secure Aggregation, 会显著减少相对于直接暴露模型更新时的服务器数据泄漏。主要方式是通过对客户端传入中央服务器的各自的本地数据集更新模型 vector 进行加密, 中央服务器再对加密向量进行Aggregation. 对于更加具体的Secure Aggregation一般是如何流程的, 我们 delay 到~\autoref{sec:Generalized Secure Aggregation Framework}

The critical role of secure aggregation occurs in step three, which distinguishes secure Federated Learning (SFL) from standard Federated Learning. In this step, secure aggregation is employed to significantly reduce the data leakage that would otherwise occur if model updates were directly exposed to the server. This is achieved by encrypting the locally updated model vectors that clients send to the central server, which then aggregates these encrypted vectors. For a more detailed discussion on the typical processes involved in secure aggregation, we refer to Section~\autoref{sec:Generalized Secure Aggregation Framework}.


\subsection{Input Validation \& Byzantine-robust}
\label{subsec:Input Validation}
% 单纯考虑非 secure 的 Aggregation 过程中 (无需加密), 由于 client的数量往往比较大, 数据交互的流程也比较复杂, 这造成最终结果性能上的很大的不确定性, 这些不确定往往是因为个别 client 上传过程中的的一些不小心疏忽, 或是有意为之(poisoning attack). 于是人们在 首先提出了可以对client 上传上来的 vector进行一些简单的条件限制(norm 限制), 可以在一定程度上环节这一问题, 然而效果并不明显. 而后人们在 Federated Learning 中提出了更复杂的Input Validation验证方法, 并可以达到所谓的Byzantine-robust 的概念. 简单来说Byzantine-robust 的 federated learning aims to enable a service provider to learn an accurate global model when a bounded number of clients are malicious. 下面我们将分别介绍已有的 非 secure 和 secure 的 Aggregation 过程中的Input Validation方法.

When considering non-secure aggregation (without encryption), the large number of clients and the complexity of data exchange processes often introduce significant uncertainty in the final model’s performance. These uncertainties can arise due to inadvertent mistakes or adversarial intentional actions, such as poisoning attacks, by individual clients during the model update process. To mitigate these issues, it is common to calculate an \textit{aggregation weight} for each client at the server to manage such risks. For example, researchers initially proposed simple constraints on the vectors uploaded by clients, such as norm bounds, where vectors with larger norms would be assigned smaller aggregation weights or might even be discarded. However, these measures have proven only moderately effective~\cite{fltrust}. Subsequently, more sophisticated input validation methods have been introduced in FL, aiming to achieve \textit{Byzantine-robustness}. In essence, Byzantine-robust Federated Learning enables a service provider to learn an accurate global model even when a bounded number of clients are malicious. Below, we introduce the existing methods for Input Validation in both non-secure and secure aggregation processes.


\para{Input Validation in  Aggregation}
% 之前FL 的 work 都是怎么进行 Input Validation 的
% FLTrust

Input Validation in Aggregation involves the implementation of techniques designed to ensure that the model updates provided by clients are both reliable and secure, thereby maintaining the performance and integrity of the global model. This is particularly important in the presence of Byzantine faults, where some clients may act maliciously or submit incorrect updates, either due to errors or deliberate intent.

Byzantine-robustness~\cite{} in this context refers to the ability of the FL system to withstand and operate effectively despite the presence of such malicious clients. The challenge lies in ensuring that the global model remains accurate and unbiased, even when a portion of the participating clients is actively attempting to compromise the training process. Various strategies have been developed to address this challenge, focusing on filtering out or mitigating the impact of potentially harmful updates.


One of the simplest forms of input validation is norm bounding~\cite{}, which involves setting limits on the $L_2$ norms of the model updates sent by clients. This approach restricts the influence of any single client on the global model, thereby reducing the risk of the model being skewed by outlier updates. However, while norm bounding is straightforward, it may not be sufficient in scenarios with more sophisticated attacks.

To address more complex threats, methods like Krum~\cite{Krum} have been proposed. Krum is an aggregation rule that evaluates the squared distance between a client’s model update and the updates from other clients. Specifically, Krum computes a score for each client by summing the distances between its update and those of the closest $n-f-2$ clients, where $f$ represents the number of potentially malicious clients. The client with the minimal score is then selected to update the global model. This method is particularly effective when the number of malicious clients is small, as it minimizes the impact of outlier updates by focusing on the consensus among the majority of clients.

Another approach is the Trimmed Mean (Trim-mean)~\cite{Trim-mean} method, which aggregates model updates in a coordinate-wise manner. For each parameter in the model, the server collects all values from the clients, sorts them, and then removes the largest and smallest values according to a trimming parameter $k$. The mean of the remaining values is used to update the global model. Trim-mean can tolerate up to 50\% of the clients being malicious, making it a robust method in scenarios with a higher proportion of adversarial clients.

Similarly, the Median method~\cite{Median} operates by sorting the values of each model parameter across all client updates. Instead of averaging the trimmed values as in Trim-mean, the median value is selected for the global model. This method is particularly simple but effective against outliers and certain types of malicious behavior, offering a balance between simplicity and robustness.


Finally, FLTrust~\cite{fltrust} is widely recognized as one of the most advanced approaches due to its incorporation of a trust bootstrapping mechanism. In FLTrust, the server utilizes a small, trusted dataset to compute a baseline model. It then evaluates the similarity between the updates from clients and this baseline model using a variant of cosine similarity, known as the \textbf{FLTrust score}. The \textit{FLTrust score} is defined as $\text{FLTrust score} = \max(0, \text{cossim}(v_{client}, v_{validate}))$, where \textit{cossim} denotes cosine similarity, $v_{client}$ represents the client’s intermediate result, and $v_{validate}$ represents the reference result computed by the server.

Only updates that closely align with the baseline are accepted, effectively filtering out potentially malicious contributions. By implementing this mechanism, FLTrust not only validates the inputs but also significantly enhances the overall robustness of the aggregation process, providing a stronger defense against Byzantine failures.



\para{Input Validation in Secure Aggregation}.
% SFL 中的 ACRON
In Secure Aggregation, the challenge of input validation is compounded by the encryption of model updates, which complicates the application of traditional validation methods like norm bounding. To tackle these challenges, recent research has focused on ensuring that the norms of encrypted vectors remain within acceptable limits. While such approaches offer a basic level of security, they often suffer from significant computational and communication overheads, limiting their practicality in large-scale deployments.

One of the earliest and still prevalent approaches is zPROBE by Ghodsi et al.~\cite{zPROBE}, which employs a generic proof framework to verify that each entry of a client’s masked input is honestly derived from an input of bounded size. However, due to the high computational cost, this method only verifies a random subset of entries. This selective verification might not be robust enough for Federated Learning (FL), where even small deviations in a few entries could compromise the entire model.

Similarly, Karakoç et al.~\cite{karakocc2021secure} have proposed a method involving secure aggregation with range validation through an oblivious programmable pseudorandom function. However, their work remains at the proof-of-concept stage, with experimental validation limited to very small vector lengths (e.g., 16), due to the prohibitive computational costs involved.

In contrast to these early-stage or computationally intensive approaches, ACORN~\cite{} has emerged as a highly efficient solution. Unlike methods that impose heavy communication costs or rely on complex cryptographic proofs, ACORN optimizes the validation process by embedding norm validation directly within the secure aggregation protocol itself. This integration allows ACORN to maintain a balance between security and efficiency, ensuring that only well-formed, legitimate updates contribute to the global model. As a result, ACORN significantly mitigates the risk of poisoning attacks while also being one of the fastest input validation methods currently available for Secure Aggregation.

On the other hand, methods like RoFL\cite{RoFL} and EIFFeL\cite{EIFFeL}, introduced by Lycklama et al. and Chowdhury et al. respectively, have focused on more complex multi-server setups. RoFL, for instance, requires each client to send commitments for every vector entry, leading to substantial communication overhead—up to 51 MB for a vector length of 262,000 when applying an $L_{\infty}$ bound. EIFFeL distributes the computational load across clients, similar to Prio, but faces scalability issues, with communication overheads increasing quadratically with the number of clients and linearly with the vector length.

The challenge of balancing input validation with communication costs continues to be a major focus in the development of Secure Aggregation protocols. While RoFL and EIFFeL offer innovative approaches, their practicality is often hindered by these overheads. In contrast, ACORN stands out as a streamlined and effective solution, particularly in scenarios where speed and efficiency are critical.


\subsection{Homomorphic Encryption}
\label{subsec:Homomorphic Encryption}
Homomorphic encryption is a class of cryptographic algorithms that allow computations to be performed directly on encrypted data without needing to decrypt it first. This means that the computing party, such as a cloud service provider, can process data while it remains encrypted, ensuring that sensitive information is never exposed in its unencrypted form. This capability is crucial in scenarios where privacy and security are paramount, such as in financial services, healthcare, and data analytics.

There are two main types of homomorphic encryption: partial homomorphic encryption (PHE) and fully homomorphic encryption (FHE). Partial homomorphic encryption supports only one type of computation, either addition or multiplication, on encrypted data, but not both. Fully homomorphic encryption (FHE) allows for arbitrary computations on encrypted data. This makes FHE a powerful tool for secure data processing, but it comes with significant computational overhead, making it more resource-intensive and slower compared to partial homomorphic encryption.

\para{PHE}.
The Naccache-Stern cryptosystem is a partial homomorphic encryption (HE) scheme that allows for homomorphic addition of ciphertexts while maintaining a reasonable level of efficiency and security. This cryptosystem operates over a composite modulus \( n = pq \), where \( p \) and \( q \) are large prime numbers. A message \( m \) is encrypted by computing the ciphertext \( c \) as:
\[
c = g^m \cdot r^n \mod n
\]
where \( g \) is a generator of a subgroup of \( \mathbb{Z}_n^* \), and \( r \) is a random value. The homomorphic property of the Naccache-Stern scheme enables the multiplication of two ciphertexts \( c_1 \) and \( c_2 \), resulting in a new ciphertext \( c_3 \) that corresponds to the sum of the original plaintexts, i.e., \( c_3 = c_1 \cdot c_2 \mod n \), which decrypts to \( m_1 + m_2 \). However, this scheme does not support homomorphic multiplication, limiting its applications to scenarios where additive operations on encrypted data are sufficient. The use of a large composite modulus \( n \) provides security against known attacks, making the Naccache-Stern cryptosystem a viable choice for applications requiring efficient homomorphic addition.


\para{FHE}.
The CKKS (Cheon-Kim-Kim-Song) protocol is a homomorphic encryption scheme tailored for performing approximate arithmetic on encrypted data, making it highly suitable for privacy-preserving computations on real or complex numbers. In this scheme, a plaintext value \( m \) is first encoded into a polynomial \( m(x) \) within the ring \( \mathbb{R}[x]/(x^n + 1) \), where \( n \) is the polynomial modulus degree. The encoded polynomial is then scaled by a factor \( \Delta \), which controls the precision of subsequent arithmetic operations. The encryption of the plaintext is expressed as:
\[
c(x) = a(x) + \Delta \cdot m(x) + e(x) \pmod{q(x)}
\]
where \( a(x) \) is a random polynomial, \( e(x) \) is an error polynomial introduced during encryption, and \( q(x) \) is the ciphertext modulus. The noise \( e(x) \), which accumulates with each homomorphic operation, necessitates careful parameter selection to balance precision, efficiency, and security within the protocol.

 
% \para{FHE.}

% \para{PHE.}


\subsection{Zero-Knowledge Proof and zk-SNARKs}
Zero-Knowledge Proof (ZKP) is a fundamental concept in cryptography that enable one party, known as the prover, to demonstrate to another party, the verifier, that they possess a certain piece of information or can perform a specific computation without revealing the actual information or details of the computation itself. This unique capability has profound implications for enhancing privacy and security in various applications, ranging from authentication systems to secure multiparty computations. The core idea behind ZKPs is to provide assurance that the prover is truthful without requiring them to disclose sensitive data, thereby preventing any potential leakage of information during the verification process.


\para{zk-SNARKs.} Zero-Knowledge Succinct Non-Interactive Arguments of Knowledge (zk-SNARKs) extend the privacy-preserving properties of ZKPs by introducing additional features such as succinctness and non-interactivity. These features allow zk-SNARKs to generate highly compact proofs that require minimal communication between the prover and verifier, significantly improving efficiency and scalability. Succinctness ensures that the proofs are short, even for complex computations, while non-interactivity eliminates the need for multiple rounds of interaction between the parties, making the protocol practical for real-world applications, including blockchain technology and privacy-preserving smart contracts. The detailed protocol of zk-SNARKs will be introduced in \autoref{subsec:zk-SNARKs Construction}.


\para{R1CS.} Rank-1 Constraint System (R1CS) is a formalism used in cryptographic proof systems, particularly in zero-knowledge proofs like zk-SNARKs. zk-SNARKs cannot directly understand a statement that the prover needs to prove, such as a complicate mathematics formula, and therefore, the statement needs to be converted into R1CS format. An R1CS represents a system of arithmetic constraints as a set of quadratic equations over a finite field. Each constraint in an R1CS takes the form $(\mathbf{A}_i \cdot \mathbf{X}) \times (\mathbf{B}_i \cdot \mathbf{X}) = (\mathbf{C}_i \cdot \mathbf{X})$ for each $i$, where $\mathbf{A}_i$, $\mathbf{B}_i$, and $\mathbf{C}_i$ are vectors of coefficients, and $\mathbf{X}$ is a vector of variables. The goal is to ensure that the product of two linear combinations of variables equals another linear combination. The entire system of constraints is designed to facilitate efficient verification of complex computations in a cryptographic context, allowing a prover to demonstrate knowledge of a valid solution (known as a witness) without revealing any private information. The R1CS framework is integral to the construction of succinct and non-interactive cryptographic proofs.




\subsection{Motivation and Challenge}
\label{subsec:Motivation and Challenge}

% Byzantine-robust federated learning aims to enable a service provider to learn an accurate global model when a bounded number of clients are malicious. 这对Federated Learning 过程中的大量不确定性(party 非常多, 计算流程复杂且分散)有很好的缓和作用. 而在 secure aggregation 的 FL 的现有研究中, 没有方案可以做到Byzantine-robust,  因为想要实现Byzantine-robust 的 secure aggregation是非常困难的, 需要对加密的 vector 进行验证. 因此现有 secure aggregation 的 Literature 中 只能做到非常简单, 且对Byzantine-robust 效果非常有限的 Input Validation, 比方说 验证 加密 vector norm 大小是否超过给定范围~\cite{ACRON}. 然而即便是这样看起来简单的 Input Validation, 在验证的 protocal 上已经非常复杂了~\cite{ACORN}. 这使得在Byzantine-robust federated learning中真正非常有效的Input Validation SOTA~\cite{FLTrust} 无法使用在Secure Aggregation 中.  出于这样的需求, 我们构造了~\ourmethod{}, 一个可以高效运行的 Byzantine-robust Secure Aggregation for federated learning, 我们使用的是Byzantine-robust federated learning中的 SOTA, FLTrust~\cite{}作为 Input Validation 的方案, 我们针对 FLTrust设计了protocal, 可以让 FLTrust 的 Validation 方案, 可以在Secure Aggregation for federated learning的场景下高效工作, 来满足Secure Aggregation for federated learning的Byzantine-robust需求.

\para{Motivation.}
Byzantine-robust federated learning aims to enable a service provider to learn an accurate global model even when a certain number of clients behave maliciously. This robustness is crucial in addressing the inherent uncertainties in the federated learning process, where numerous parties are involved, and the computation is complex and distributed. However, in the context of secure aggregation within federated learning, there is currently no method that achieves Byzantine robustness. Achieving Byzantine-robust secure aggregation is particularly challenging because it requires validating encrypted vectors, which complicates the process significantly.

Existing literature on secure aggregation has only managed to implement very basic forms of input validation, such as verifying whether the norm of an encrypted vector stays within a predefined range~\cite{ACORN}. Despite being seemingly simple, even these basic validation methods necessitate highly complex protocols~\cite{ACORN}. As a result, state-of-the-art (SOTA) input validation methods that are highly effective in Byzantine-robust federated learning, such as FLTrust~\cite{}, cannot be directly applied in the secure aggregation context.

To address this need, we propose~\ourmethod{}, an efficient Byzantine-robust secure aggregation method for federated learning. Our approach leverages FLTrust, the SOTA method in Byzantine-robust federated learning, as the input validation technique. We have specifically designed a protocol that allows FLTrust’s validation mechanism to operate efficiently within the secure aggregation framework, thus fulfilling the Byzantine robustness requirements for secure federated learning.


% 
% 正如上面所说, 想要实现Byzantine-robust 的 secure aggregation是困难的. 这主要体现在从原本的验证明文的 vector (Byzantine-robust federated learning ), 转换成了验证密文的 vector (Byzantine-robust secure federated learning).  验证密文的方式取决于加密方案, 前文提到一般来说加密方案可被大体分为两类, PHE 和 FHE, 两者在速度和 operator 的使用范围之间各有优缺点. 现有 Byzantine-robust federated learning 的 SOTA 方案如 FLTrust, 需要对 vector 进行 max(a,b), 以及 cos similarity 这样比较复杂的 operator操作,  如果使用 FHE, 虽然加密 vector可以直接使用这些复杂的 operator操作, 但是效率往往比 PHE 慢上 100 倍甚至更多~\cite{},这往往造成运算时间超出合理范围.而如果使用PHE, 加密向量将只能使用加法来满足本身 aggregation 这个一定必须的过程, 而在无法使用其他 operator 的情况下, 需要设计非常复杂的 protocal,  但却可以让运算时间处于合理范围. 一个典型的例子是, Previous study ACRON~cite{ACRON}(published in USENIX security 2023, Security 领域的顶会) 仅验证了加密 vector 的 norm 会不会超过一个固定值, protocal 就已经非常复杂了. 但却可以保证验证的高效性. 然而 仅仅验证vector 的 norm 会不会超过一个固定值是远远无法达到Byzantine-robust的目的的. 所以想要实现Byzantine-robust 的 secure aggregation是困难的 有显著 gap 的.
\para{Challenges}.
As mentioned above, achieving Byzantine-robust secure aggregation is a significant challenge. The primary difficulty lies in transitioning from validating plaintext vectors, as done in Byzantine-robust federated learning, to validating encrypted vectors in the context of secure federated learning. The method of validation depends heavily on the encryption scheme used. Generally, encryption schemes can be categorized into two types: PHE and FHE, each with its own trade-offs in terms of speed and the range of operators available.

State-of-the-art Byzantine-robust federated learning methods, like FLTrust, require complex operations on vectors, such as max(a, b) and cosine similarity. Using FHE allows these operations to be directly applied to encrypted vectors, but at a significant cost: FHE is often 100 times slower than PHE~\cite{}, which can make the computation time impractical. On the other hand, PHE supports only basic operations like addition, which is necessary for aggregation but insufficient for more complex validations. Therefore, while PHE can be more efficient, it requires designing very sophisticated protocols to work around its limitations.

A notable example is the ACORN protocol~\cite{ACORN}, published in USENIX Security 2023, which focuses solely on validating whether the norm of an encrypted vector exceeds a fixed threshold. Even this relatively simple validation task requires a highly intricate protocol to ensure efficiency. However, merely validating the norm of a vector is far from sufficient to achieve Byzantine robustness.

Thus, the gap between current capabilities and the goal of achieving Byzantine-robust secure aggregation remains substantial, presenting a significant challenge for further research and development.








==> old/3.tex <==
\section{Preliminary}
\label{sec:Preliminary}



\subsection{Threat Model}
\label{subsec:Threat Model}

\para{Overall Setup.}
% 我们考虑一共有 n 个 clients, 意图在 privacy-perserving 的 manner (privacy leakage analysis 在 section~\ref{}) 下  一同开发一个可以参数开源的模型.  一个 central server $\mathbb{S}_C$ 负责接收每个 client 发送过来的经过加密了的 private vector $\mathcal{E}(\mathbf{\beta}_{\mathbf{i}}) \in \mathbb{Z}_t^{\ell}$, 其中$\mathcal{E}(\cdot)$ 表示加密算法,   $\mathbf{\beta}_{\mathbf{i}}$ 表示第$i$个 client 的 private vector. 其中加密算法和加密算法的秘钥是由 confidential encryptal server $\mathbb{S}_E$ 提供. 这里我们假设 $\mathbb{S}_E$ 是 独立于 $\mathbb{S}_C$ 的机构, 意味着$\mathbb{S}_E$ 不会与$\mathbb{S}_C$串通. 这样的假设一方面符合真实应用场景, 比方说 xxxx, 另一方面, 这样独立的两个 server 可以更高效, 更低 Privacy Leakage 的前提下地使得最终的模型可以以明文形式 open source; $\mathbb{S}_C$只负责对 client 上传上来的加密向量进行 aggregation, 在 Privacy 方面不会有信息泄露, 效率方面由于 server 仅仅是 aggregation, 加密算法可以使用 partial HE, 大大提升效率. 而$\mathbb{S}_E$方面, 如果模型仅聚合一次, $\mathbb{S}_E$获得的隐私信息等同于最终参数开源后所有人能够得到的信息, 而如果模型聚合多次, $\mathbb{S}_E$也仅仅只是得到多次聚合过程中, 未完全优化好的模型参数, 单个 client 隐私的泄露也是可以被控制在合理范围, 尤其是在 client 数量大的情况下. 这样的做的好处是最终的模型将可以不再是密文形式保存~\ref{}, 而是可以对参数进行开源~\ref{}.符合了当今AI 领域对于 Open source的诉求. 
We consider a scenario involving $n$ clients who intend to collaboratively develop an open-source model in a privacy-preserving manner (as analyzed in Section~\ref{}). A central server, denoted as $\mathbb{S}_C$, is responsible for receiving encrypted private vectors $\mathcal{E}(\mathbf{\beta}_{\mathbf{i}}) \in \mathbb{Z}_t^{\ell}$ from each client, where $\mathcal{E}(\cdot)$ represents the encryption algorithm, and $\mathbf{\beta}_{\mathbf{i}}$ represents the private vector of the $i$th client. The encryption algorithm and its keys are provided by a confidential encryption server, $\mathbb{S}_E$, which is assumed to be independent of $\mathbb{S}_C$. This assumption ensures that $\mathbb{S}_E$ does not collude with $\mathbb{S}_C$. Such an assumption is realistic in many scenarios, such as [example scenarios], and facilitates the development of a plaintext model that can be open-sourced with greater efficiency and minimal privacy leakage. $\mathbb{S}_C$ is only responsible for aggregating the encrypted vectors uploaded by the clients, ensuring no privacy is compromised at this stage. The use of partial homomorphic encryption (HE) allows for enhanced efficiency during aggregation. On the other hand, $\mathbb{S}_E$ has access only to information equivalent to the final open-source parameters if the model is aggregated once. If multiple rounds of aggregation are performed, $\mathbb{S}_E$ gains access to intermediate, non-optimized model parameters. The privacy leakage for any individual client remains within reasonable bounds, especially when the number of clients is large. The benefit of this approach is that the final model can be openly shared as plaintext parameters rather than encrypted, aligning with the AI community's growing demand for open-source contributions (Section~\ref{}).


\para{Client Goals and Capabilities.}
% 我们假设大部分 client 是会 honest 会 follow instruction 做出最终的模型. 会有不 honest的 client, 他们either 由于  accidental or 会出于希望最终的模型的 bias 会更偏好对自己的数据表现更好而可能修改 data 或修改 自己的 aggregation weight. 我们假设只有部分 client 可能会有这种 dishonest 行为, 因为如果所有或大部分 client 都不 honest, 这种情况下模型也是无法训练的. ~\ourmethod的目的也是希望通过 ZKP 排查出这种client.
We assume that the majority of clients will act honestly and follow instructions to contribute to the final model. Clients have control over the encrypted vectors they send to $\mathbb{S}_C$, the aggregation weights they use, and the generation of ZKP proofs. However, we also consider the possibility of some clients being dishonest. These dishonest clients might modify their data or alter their aggregation weights, either accidentally or in an attempt to bias the final model in favor of their own data. We assume that only a subset of clients may engage in such dishonest behavior, as the model cannot be effectively trained if most or all clients act dishonestly. The goal of our method is to leverage ZKP to identify and eliminate such clients.




\para{$\mathbb{S}_E$ and $\mathbb{S}_C$ Assumptions.}  
% 我们假设$\mathbb{S}_E$ 与 $\mathbb{S}_C$ 都是没有恶意的, 然而我们在~\ref{subsec:Privacy and Security Analysis}中, 对 $\mathbb{S}_E$ 与 $\mathbb{S}_C$的潜在恶意行为会对 Security 和 Privacy 带来的伤害进行了分析.
Both $\mathbb{S}_E$ and $\mathbb{S}_C$ are assumed to be non-malicious. However, in Section~\ref{subsec:Privacy and Security Analysis}, we analyze the potential security and privacy risks associated with malicious behavior by $\mathbb{S}_E$ and $\mathbb{S}_C$.

% aaaa


\subsection{Definition and Notation}
% m个 party, 
 Initial Global Model parameter: $\beta_0$ \\
 validation dataset intermediate result: $\beta*$ \\%-> v0
 ith client intermediate result: $\beta_i$ \\%-> v1
 ith client Aggregation weight: $\alpha_i$ \\% alpha
 ith client local update: $\hat\beta_i = \alpha_i * \beta_i$ \\%-> v1
 Final Global Model parameter : $\hat\beta = \frac{\sum_i^m \hat\beta_i}{m} $ %-> 



==> old/To-do.tex <==
% 1. 服务器将 $\beta^*$ 明文分享给客户端。这是否合理？如果服务器的数据是私有的呢？
% 在 Threat model 里进行说明

% 2*. 所实现的协议似乎与原始的 FLTrust 方法不同。缺少两个步骤：1. 在与信任分数相乘之前对梯度进行归一化。2. 使用信任分数作为权重进行加权平均，这与加权求和不同。(The implemented protocol seems to be different from the original FLTrust approach. Two missing steps: 1. Normalization of gradient before multiplying with trust score. 2. Weighted *averaging* with trust scores as weights, which is different from a weighted *sum*.)
% (1). 在 client 端添加归一化
% (2). 该对应的 第5章

% 3. 在多个地方，FedAvg 被描述为一种 “meta-analysis” 方法，并且只需要一个聚合轮次。我认为这不准确。FedAvg 是为多轮次应用而设计的。
% 修改 FedAvg 的引用


% 4. 此外，有一些关于此工作的声明，声称它允许最终模型以私有方式发布而不泄露其他任何信息。这在标准的多轮设置中是否仍然适用？单轮聚合的联邦学习听起来不太现实。
% 


% 5. 您所提到的 “secure federated learning” 是指哪一组工作？我想知道您是否特指 Secure Aggregation（如 https://arxiv.org/abs/1611.04482 中的概念）。如果每轮更新的聚合后仍然解密并应用于模型，我个人认为这不能称为 “secure federated learning”。除非您看到许多论文都这样使用这个术语。“Secure” 这个词被广泛使用，应该谨慎使用，以免引入更多混淆。
% 1)每轮更新的聚合后仍然解密并应用于模型依然叫Secure fl 的文章引用
%    VerifyNet: Secure and Verifiable Federated Learning
%    FEDERATED LEARNING WITHOUT REVEALING THE DECISION BOUNDARIES
%    Secure Federated Learning with a Homomorphic Encryption Model

% 6. 值得将基于 HE 的安全聚合方法与上述链接中的其他提议区分开来。这可以根据执行加密计算的需求进行合理化，以实现 FLTrust 等鲁棒性措施。(It would be worth distinguishing the HE-based approach to secure aggregation from other proposals like the above link. Could be justified based on the need to perform encrypted computation for robustness measures like FLTrust.)

% 7. 在某些地方，$\alpha$ 的定义似乎不一致。请参见第 9 页协议中的 $\beta^*$ 和第 10 页文本中的 $\beta_\text{hat}$。

% 8. 请澄清 $\beta^*$ 是否在 zk-SNARK 中被视为私有输入，因为它对服务器和客户端都是已知的。(Clarify whether beta* is considered private input in zk-SNARK, since it's known to both the server and the client.)

% 9. 对于 Baseline MHE 协议，服务器应使用明文的 $\beta^*$ 而非加密的，以显著加快速度。另外，需要澄清使用了哪种方法来近似 max 函数，因为这不是标准的同态运算。设置步骤需要更新，以删除与客户端共享 $\beta^*$，这是不必要的。

% 10. 请澄清实验中使用的 CKKS 参数，这对运行时间有很大影响。这些参数需要根据协议的复杂性选择，以避免不必要的开销。

% 11. 澄清选择 PHE 方案的原因。为什么不选择 Paillier，我认为这更常见？根据我所见，它们似乎关系密切。

% 12. 需要澄清 $\beta_i$ 本身的正确性并未得到保证。客户端仍然可以发送任意模型更新。确切的保证是 FLTrust 方案已正确应用于提交的加密更新中。

% 13. 为了更广泛地框定贡献，提及除 FLTrust 之外可以使用相同技术支持的其他方法。

==> tablecopy.tex <==
\section{Implementation and Evaluation}



\subsection{Evaluation}
To demonstrate the effectiveness of our scheme, we conducted several experiments to evaluate the overall performance and actual runtime of each component.

\para{Client.} Each client follows three major steps. First, the client computes their own $\alpha$ for cosine similarity and calculates the vector $v1_a = v_1 \times \alpha$. Next, they encrypt each data point in the vector using homomorphic encryption, which can then be sent to the server later. Finally, the client uses zk-SNARKs to prove that the vector they sent to the server was correctly computed with $\alpha$. Since the computation of $v1_a$ is performed on unencrypted data before applying homomorphic encryption, this step is computationally efficient. The majority of the client’s time is consumed by zk-SNARKs proof generation and the homomorphic encryption process. Cryptographic algorithms are designed to process data in fixed-size blocks or using a consistent set of operations, ensuring that the computational effort remains constant regardless of the actual values within the data. This consistency is crucial for maintaining security, as it prevents timing attacks, where an attacker could infer information about the input based on variations in encryption time. Therefore, the encryption time depends only on the size of the vector, regardless of the actual values within it. Consequently, under the same vector size, each client should require a similar amount of time to complete their steps.

\para{Server 1.}
Recall that Server 1 does not possess the private (decryption) key. Its tasks are limited to computing the sum of all vectors it receives from the clients and verifying the zk-SNARKs proofs provided by the clients. Therefore, the time cost for Server 1 depends on the number of clients and the size of the vectors.

\para{Server 2.}
Server 2 is responsible for decrypting the vectors using its private (decryption) key. Since the number of clients does not affect the size of the vectors, the time cost for Server 2 depends solely on the size of the vectors.

\subsection{Performance Affect Based on Bit Length Size}

First, we evaluate the end-to-end performance of our model with varying vector sizes. In our setup, the server receives data from two clients. The full FLTrust model comprises a vector containing 1,663,370 elements. Additionally, we modify the FLTrust model’s data structure to assess the performance of our scheme with different vector lengths. Table \ref{tab:vector_length} presents the evaluation results for each step in our model.

\begin{table*}[]
\centering
\begin{tabular}{c|c||cccccc}
\hline
\multirow{2}{*}{Scheme} & \multirow{2}{*}{Step} & \multicolumn{5}{c}{Beta Length}                                                                               \\ \cline{3-8} 
                      & & \multicolumn{1}{c|}{58252} & \multicolumn{1}{c|}{110030} & \multicolumn{1}{c|}{213586} & \multicolumn{1}{c|}{420698} & \multicolumn{1}{c|}{834922} & 1663370 \\ \hline\hline
\multirow{8}{*}{PHE} & Client Compute        & \multicolumn{1}{c|}{0.60}  & \multicolumn{1}{c|}{0.66} & \multicolumn{1}{c|}{0.73}  & \multicolumn{1}{c|}{0.93}& \multicolumn{1}{c|}{1.36}      & 1.81 \\ \cline{2-8}
& Client Encrypt        & \multicolumn{1}{c|}{82.11}  & \multicolumn{1}{c|}{174.50} & \multicolumn{1}{c|}{305.71}  & \multicolumn{1}{c|}{601.41}& \multicolumn{1}{c|}{1188.92}      & 2340.36 \\ \cline{2-8}
& Client Prove          & \multicolumn{1}{c|}{0.99}  & \multicolumn{1}{c|}{1.27} & \multicolumn{1}{c|}{2.03}  & \multicolumn{1}{c|}{3.42}& \multicolumn{1}{c|}{5.04}      & 8.43 \\ \hhline{~|=======}
& Server 1 Compute      & \multicolumn{1}{c|}{0.31}  & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{1.09}  & \multicolumn{1}{c|}{2.16}& \multicolumn{1}{c|}{4.31}      & 8.98 \\ \cline{2-8}
& Server 1 Verify       & \multicolumn{1}{c|}{0.79}  & \multicolumn{1}{c|}{0.75} & \multicolumn{1}{c|}{0.74}  & \multicolumn{1}{c|}{0.74}& \multicolumn{1}{c|}{0.76}      & 0.73 \\ \hhline{~|=======}
& Server 2 Decrypt      & \multicolumn{1}{c|}{84.39}  & \multicolumn{1}{c|}{176.13} & \multicolumn{1}{c|}{308.26}  & \multicolumn{1}{c|}{605.64}& \multicolumn{1}{c|}{1248.08}      & 2471.44 \\ \cline{2-8}
% Server 2 Compute      & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s} & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}& \multicolumn{1}{c|}{1s}      & 1s \\ \hline\hline
& Total      & \multicolumn{1}{c|}{172.48}  & \multicolumn{1}{c|}{354.01} & \multicolumn{1}{c|}{618.50}  & \multicolumn{1}{c|}{1214.30}& \multicolumn{1}{c|}{2450.62}      & 4839.45 \\ \hline\hline

\multirow{5}{*}{FHE} & Client Compute        & \multicolumn{1}{c|}{0.58}  & \multicolumn{1}{c|}{0.61} & \multicolumn{1}{c|}{0.63}  & \multicolumn{1}{c|}{0.75}& \multicolumn{1}{c|}{1.02}      & 1.55 \\ \cline{2-8}
& Client Encrypt        & \multicolumn{1}{c|}{563.18}  & \multicolumn{1}{c|}{1063.77} & \multicolumn{1}{c|}{2106.89}  & \multicolumn{1}{c|}{3942.43}& \multicolumn{1}{c|}{7590.36}      & 14516.98 \\ \hhline{~|=======}
& Server 1 Compute      & \multicolumn{1}{c|}{5170.23}  & \multicolumn{1}{c|}{9472.45} & \multicolumn{1}{c|}{18380.68}  & \multicolumn{1}{c|}{36102.05}& \multicolumn{1}{c|}{>12h}      & >12h \\ \hhline{~|=======}
& Server 2 Decrypt      & \multicolumn{1}{c|}{178.13}  & \multicolumn{1}{c|}{331.58} & \multicolumn{1}{c|}{611.47}  & \multicolumn{1}{c|}{1143.30}& \multicolumn{1}{c|}{n/a}      & n/a \\ \cline{2-8}
% Server 2 Compute      & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s} & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}& \multicolumn{1}{c|}{1s}      & 1s \\ \hline\hline
& Total      & \multicolumn{1}{c|}{5913.28}  & \multicolumn{1}{c|}{10871.74} & \multicolumn{1}{c|}{21103.23}  & \multicolumn{1}{c|}{41190.88}& \multicolumn{1}{c|}{>12h}      & >12h \\ \hline

\end{tabular}
\caption{Beta Length}
\label{tab:vector_length}
\end{table*}

\subsection{Performance Affect Based on Number of Client}
As the number of clients increases, the server is required to perform more computations on encrypted data using homomorphic encryption. Additionally, it must verify a greater number of zk-SNARK proofs, which can significantly impact the overall runtime for the server. These increased computational demands can lead to higher runtime, and to gain a deeper understanding of the time performance of our model with varying numbers of clients, we conducted a comprehensive evaluation. This evaluation aims to assess how the server’s processing time are affected as the number of clients increases. We set the vector size as 58252 by adjust the FLTrust model shape, and Table \ref{tab:client_number} shows our evaluation results with 2, 4, 8, 16, 32, 64, and 128 clients.




\begin{table*}[]
\centering
\begin{tabular}{c|c||ccccccc}
\hline
\multirow{2}{*}{Scheme} & \multirow{2}{*}{Step} & \multicolumn{7}{c}{Client Size}                                                                                                                                                     \\ \cline{3-9} 
                      & & \multicolumn{1}{c|}{2}  & \multicolumn{1}{c|}{4}  & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{32} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c}{128} \\ \hline\hline
\multirow{3}{*}{PHE} & Server 1 Compute      & \multicolumn{1}{c|}{0.32} & \multicolumn{1}{c|}{0.64} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{2.49} & \multicolumn{1}{c|}{5.27} & \multicolumn{1}{c|}{9.88} & 18.07                       \\ \cline{2-9} 
& Server 1 Verify       & \multicolumn{1}{c|}{0.78} & \multicolumn{1}{c|}{1.51} & \multicolumn{1}{c|}{2.96} & \multicolumn{1}{c|}{5.89} & \multicolumn{1}{c|}{11.84} & \multicolumn{1}{c|}{23.69} & 47.29                       \\ \cline{2-9} %\noalign{\vskip\doublerulesep  \vskip-\arrayrulewidth}  \cline{2-9} 
& Server 2 Decrypt      & \multicolumn{1}{c|}{85.78} & \multicolumn{1}{c|}{82.54} & \multicolumn{1}{c|}{85.19} & \multicolumn{1}{c|}{85.64} & \multicolumn{1}{c|}{84.15} & \multicolumn{1}{c|}{84.97} & 85.22                       \\ \hline\hline

\multirow{2}{*}{FHE} & Server 1 Compute      & \multicolumn{1}{c|}{5172.77} & \multicolumn{1}{c|}{8516.44} & \multicolumn{1}{c|}{14924.16} & \multicolumn{1}{c|}{29067.35} & \multicolumn{1}{c|}{57791.80} & \multicolumn{1}{c|}{112513.73} & 218008.11                       \\ \cline{2-9}%\noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}  \cline{2-9} 
& Server 2 Decrypt      & \multicolumn{1}{c|}{1741.73} & \multicolumn{1}{c|}{1748.34} & \multicolumn{1}{c|}{1745.72} & \multicolumn{1}{c|}{1739.91} & \multicolumn{1}{c|}{1745.13} & \multicolumn{1}{c|}{1740.12} & 1746.27                      \\ \hline
\end{tabular}
\caption{Client}
\label{tab:client_number}
\end{table*}


\subsection{Transmission Cost of the Scheme}
Since our scheme involves interaction between the client, Server 1, and Server 2, the size of the data transmission is also a critical factor, as large transmissions can result in increased latency. To assess this aspect, we conducted an additional experiment to evaluate the transmission cost within our scheme. Specifically, we measured the cost for data sent from each client to Server 1, from Server 1 to Server 2, and from Server 2 back to each client. Recall that the number of clients does not affect the size of the vector that Server 1 transmits to Server 2. Therefore, our experiment focuses on evaluating how transmission costs vary with different vector sizes. Table \ref{tab:transmission} show the transmission cost for each party including the size of zk-SNARKs proof and the vector.


\begin{table}[]
\begin{tabular}{c|c||ccccc}
\hline
\multirow{2}{*}{Transmission}         & \multirow{2}{*}{Cost} & \multicolumn{5}{c}{Beta Length}                                                                                 \\ \cline{3-7} 
                                      &                       & \multicolumn{1}{c|}{100} & \multicolumn{1}{c|}{1K}  & \multicolumn{1}{c|}{10K} & \multicolumn{1}{c|}{100K} & 1M  \\ \hline\hline
\multirow{2}{*}{\makecell[c]{Client to \\Server 1}}   & Size                  & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB}  & 1MB \\ \cline{2-7} 
                                      & Time                  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}   & 1s  \\ \hline
\multirow{2}{*}{\makecell[c]{Server 1 to \\ Server 2}} & Size                  & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB}  & 1MB \\ \cline{2-7} 
                                      & Time                  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}   & 1s  \\ \hline
\multirow{2}{*}{\makecell[c]{Server 2 \\ to Client}}   & Size                  & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB} & \multicolumn{1}{c|}{1MB}  & 1MB \\ \cline{2-7} 
                                      & Time                  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}  & \multicolumn{1}{c|}{1s}   & 1s  \\ \hline
\end{tabular}
\caption{transmission cost}
\label{tab:transmission}
\end{table}
